SlackBench: Benchmarking Agents on Collaborative Projects Grounded in Real Code Repositories

AI Agents are becoming digital coworkers that can browse the web, write code, run experiments, and assist humans over extended horizons. Yet existing benchmarks fall short of real knowledge work: many rely on synthetic data or isolated tasks, missing the complex, multi-party dynamics of collaborative projects, where critical information is scattered across conversations, code, and evolving decisions. Even simple workplace questions may require locating relevant channels and direct messages, recovering context from long discussions, inspecting repository state, reconciling stale or conflicting evidence, and synthesizing across sources. We introduce SlackBench, a benchmark for evaluating agents on realistic research and engineering workflows that require joint reasoning over workplace communication and evolving repository state. Grounded in privacy-preserving reenactments of real academic research projects, SlackBench provides reproducible environments with realistic multi-party dialogue, evolving decisions, and corresponding code changes grounded in GitHub repositories and Google Docs. It contains 140 queries spanning heterogeneous-source agentic search, abstention on unanswerable or false-premise questions, goal-directed summarization, and circumstance inference over long conversations. These tasks are not reducible to static corpus question answering: agents must determine which conversations matter, traverse threads, inspect repository state, and synthesize evidence across communication and code artifacts. Across 33 frontier models and agent harnesses, the best system scores around 80% and most agents score below 66%, highlighting substantial headroom for improvement. SlackBench thus provides an extensible framework for evaluating agents in collaborative work environments. The SlackBench dataset is available at https://huggingface.co/datasets/HuanzhiMao/SlackBench .

==> packages.tex <==
%%==================== Math ====================
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{mathtools}                % 必须在 amsmath 之后
\RequirePackage{bm}                       % commands.tex 的 \vzero 等依赖
\RequirePackage{mathpazo}

%%==================== 排版 / 字体 ====================
\RequirePackage{microtype}
\RequirePackage{anyfontsize}
\RequirePackage{titlesec}
\RequirePackage{tocloft}
% Headings and author metadata use the same Palatino family as the body.

%%==================== 颜色 ====================
\RequirePackage{xcolor}
\RequirePackage{colortbl}
%% ---- Google GM2 palette (single source; see CLAUDE.md "Color palette") ----
\definecolor{gblue}{HTML}{1A73E8}     % blue 600
\definecolor{gred}{HTML}{D93025}      % red 600
\definecolor{gyellow}{HTML}{E37400}   % yellow 900, the only Google yellow at 3:1 on white
\definecolor{ggreen}{HTML}{1E8E3E}    % green 600
\definecolor{gpurple}{HTML}{9334E6}   % purple 600
\definecolor{ggrey}{HTML}{5F6368}     % grey 700
\colorlet{linkcol}{gblue}

%%==================== 图与排版插入 ====================
\RequirePackage{graphicx}
\RequirePackage{wrapfig}
\RequirePackage{adjustbox}
\RequirePackage{tikz}                     % \circled 依赖

%%==================== Caption ====================
\RequirePackage[labelsep=colon]{caption}
\RequirePackage{subcaption}               % 必须在 caption 之后

%%==================== 表格 ====================
\RequirePackage{booktabs}
\RequirePackage{multirow}
\RequirePackage{tabularx}
\RequirePackage{makecell}

%%==================== 布局 ====================
\RequirePackage{geometry}
\RequirePackage{fancyhdr}
\RequirePackage{authblk}
\RequirePackage{enumitem}
\RequirePackage{tcolorbox}

%%==================== 工具 ====================
\RequirePackage{verbatim}
\RequirePackage{pifont}

%%==================== 算法 ====================
\RequirePackage[ruled,vlined,linesnumbered]{algorithm2e}
\RequirePackage{minted}                   % 需 -shell-escape

%%==================== Bib ====================
\RequirePackage[numbers,sort&compress]{natbib}

%%==================== Hyperref（必须最后加载）====================
\RequirePackage[colorlinks=true,allcolors=linkcol]{hyperref}
\RequirePackage[capitalize,noabbrev]{cleveref} % 必须在 hyperref 之后

